Reverse mathematics of rings

Using the tools of reverse mathematics in second-order arithmetic, as developed by Friedman, Simpson, and others, we determine the axioms necessary to develop various topics in commutative ring theory. Our main contributions to the field are as follows. We look at fundamental results concerning primary ideals and the radical of an ideal, concepts previously unstudied in reverse mathematics. Then we turn to a fine-grained analysis of four different definitions of Noetherian in the weak base system $\mathsf{RCA}_0 + \mathsf{I}\Sigma_2$. Finally, we begin a systematic study of various types of integral domains: PIDs, UFDs and B\'ezout and GCD domains.

==> Chapters/0-todo.tex <==
%%  TO DO  (remove later)

%\comment
{
\section*{To do}
\thispagestyle{empty}

\begin{itemize}
    \item Finish proof of Theorem \ref{thm:accp->irr-fact}: Masters > Meetings > 28/7
    
    
%    \item Finish proof of Proposition \ref{prop:pid-polynom}: lexicographic ordering?
    
    
%    \item Sort out Lemma \ref{lem:nfin}: Masters > Meetings > 28/7
% \end{itemize}


% \section*{Math stuff to think about}
% \begin{itemize}
    
    
%    \item Determine strength of ``every non-field PID has a proper / maximal / prime / radical / minimal prime / principal / finitely gen ideal'' - $\WKL$?
    
    
    
    
    
%    \item Reversal of Theorem \ref{thm:d1n->d1acc}: construct a computable ring $R$ with a uniformly computable, nonstabilising chain of ideals $I_0 \subseteq I_1 \subseteq I_2 \subseteq \cdots$, such that every non-finitely-generated ideal $J \subseteq R$ computes $\varnothing'$. \href{https://www.math.csi.cuny.edu/~conidis/papers/CONIDIS_VEC.pdf#page=14}{\color{blue}Conidis} \href{https://www.math.csi.cuny.edu/~conidis/papers/CONIDIS_CHAINS.pdf#page=22}{\color{dgreen}Conidis}
%    \begin{itemize}
%        \item Localisation of $\Z[\bar{x}]$ at $\{ x_n : n \in A \}$, i.e. $\loc{ \Z[\bar{x}] }{ \{ x_n : n \in A \} }$
%    \end{itemize}
    

\comment{
    \item Reversal of Theorem \ref{thm:aca-prime-princ} (prime ideals principal $\implies$ PID) ???
    
    
    \item Motzkin's characterisation of (transfinite) Euclidean domains
    
    
    \item Check existing results on Noetherian rings (e.g. Conidis) and see if the complexity can be reduced with a different notion of Noetherian
    \begin{itemize}
        \item Hilbert basis theorem: if $R$ Noetherian then $R[X]$ is Noetherian. \cite{simpson_ordinal_1988}
    
        \item Every Artinian ring is Noetherian \cite{conidis_chain_2010, conidis_computability_2019}
        
        \item If $R$ is Artinian and $\sqrt{0} \subseteq R$ exists, then $R / \sqrt{0}$ is Noetherian \cite{conidis_chain_2010}
        
        \item Every local Artinian ring is Noetherian \cite{conidis_computability_2019}

        \item Every Noetherian ring has only finitely many minimal prime ideals. \cite{conidis_computability_2021}
    \end{itemize}
    
    
    \item \Bez\ and GCD domains:
    \begin{itemize}
%    \item \Bez $\implies$ GCD domain $\implies$ AP domain
    \item \Bez $\iff$ Pr\"ufer and GCD
    \item TFAE for a GCD domain: UFD, a.c.c.p, Noetherian, atomic.
    \item TFAE for a \Bez\ domain: PID, Noetherian, UFD, a.c.c.p., atomic.
    \item GCD $\implies$ Schreier
    \end{itemize}


    \item Discrete valuation ring: many \ulink{https://en.wikipedia.org/wiki/Discrete_valuation_ring}{equivalent definitions}
    \begin{itemize}
        \item Localisation of Dedekind domain at prime ideal is a DVR

        \item $R$ field iff $R[[x]]$ DVR iff $R[[x]]$ PID
    \end{itemize}
    
    
    \item Turning UFDs into PIDs: \url{https://math.colorado.edu/~kearnes/Papers/UFDfin.pdf} or \url{https://mathoverflow.net/a/320554/136473}
    
    
    \item Show $\ACA$ equivalent to existence of factorisation functions / UFD norms
    
    
    \item PID $\iff$ Dedekind domain and UFD
    
    
    \item \url{https://math.stackexchange.com/questions/1684869/a-noetherian-integral-domain-is-a-ufd-iff-fg-is-principal}
    
    
    \item Study \ulink{https://en.wikipedia.org/wiki/Unique_factorization_domain\#Equivalent_conditions_for_a_ring_to_be_a_UFD}{equivalent defns of UFD}
    
    
    \item In PIDs: show the following reverse over $\RCA$: every non-field PID has a proper / maximal / prime / radical / minimal prime / principal / finitely gen / ideal
}

\end{itemize}


\pagebreak
}
